On the Use of External Data for Spoken Named Entity Recognition

Spoken language understanding (SLU) tasks involve mapping from speech audio signals to semantic labels. Given the complexity of such tasks, good performance might be expected to require large labeled datasets, which are difficult to collect for each new task and domain. However, recent advances in self-supervised speech representations have made it feasible to consider learning SLU models with limited labeled data. In this work we focus on low-resource spoken named entity recognition (NER) and address the question: Beyond self-supervised pre-training, how can we use external speech and/or text data that are not annotated for the task? We draw on a variety of approaches, including self-training, knowledge distillation, and transfer learning, and consider their applicability to both end-to-end models and pipeline (speech recognition followed by text NER model) approaches. We find that several of these approaches improve performance in resource-constrained settings beyond the benefits from pre-trained representations alone. Compared to prior work, we find improved F1 scores of up to 16%. While the best baseline model is a pipeline approach, the best performance when using external data is ultimately achieved by an end-to-end model. We provide detailed comparisons and analyses, showing for example that end-to-end models are able to focus on the more NER-specific words.

==> tables/all_res.tex <==
% \begin{table*}[]
% \centering
% \begin{tabular}{c|cc|cc|cc|cc}
% \hlineB{2}
% \multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{2}{c|}{\multirow{2}{*}{External data type}} &\multicolumn{2}{c|}{\multirow{2}{*}{Re-train}} & \multicolumn{4}{c}{External data size} \\
% \cline{6-9}
% \multicolumn{1}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} &\multicolumn{2}{c|}{100h} & \multicolumn{2}{c}{500h} \\
% \cline{2-9}
% \multicolumn{1}{c|}{} & Speech & \multicolumn{1}{c|}{Text} & LM & \multicolumn{1}{c|}{Model}& F1 & \multicolumn{1}{c|}{F1-label} & F1 & F1-label \\
% \hlineB{2}
% \multirow{3}{*}{ST} & \multirow{3}{*}{\cmark} & \multirow{3}{*}{\xmark} & \cmark & \xmark  & 62.8 & 71.7 & 63.6 & 72.7 \\
%  & & & \xmark & \cmark  & 63.5 & 71.9 & 64.5 & 73.2 \\
%  & & & \cmark & \cmark  & 65.8 & 73.3 & 66.1 & 74.7 \\
% \hlineB{2}
% \multirow{3}{*}{KD-ppl} & \multirow{3}{*}{\cmark} & \multirow{3}{*}{\xmark} & \cmark & \xmark  & 65.2 & 74.3 & 65.5 & 75.5 \\
%  & & & \xmark & \cmark  & 66.2 & 76.1 & 68.2 & 77.5 \\
%  & & & \cmark & \cmark  & 69.1 & 78.2 & 69.4 & 79.3 \\
% \hlineB{2}
% \multirow{3}{*}{KD-nlp} & \xmark & \cmark & \cmark & \xmark  & 67.0 & 74.4 & 68.2 & 75.9 \\
% \cline{2-9}
%  & \multirow{2}{*}{\cmark} & \multirow{2}{*}{\cmark} & \xmark & \cmark  & 69.9 & 80.4 & 72.7 & 82.1 \\
%  & & & \cmark & \cmark  & 74.6 & 82.3 & 76.6 & 83.5 \\
% \hlineB{2}
% ASR-NER & \cmark & \cmark & N/A & \cmark  & 65.7 & 74.6 & 67.1 & 76.2 \\
% \hlineB{2}
% \end{tabular}
\begin{table*}[]
\centering
\begin{tabular}{c|cc|cc|cc|cc}
\hlineB{2}
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{2}{c|}{\multirow{2}{*}{External data type}} &\multicolumn{2}{c|}{\multirow{2}{*}{Re-train}} & \multicolumn{4}{c}{External data size} \\
\cline{6-9}
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{} &\multicolumn{2}{c|}{100h} & \multicolumn{2}{c}{500h} \\
\cline{2-9}
\multicolumn{1}{c|}{} & Speech & \multicolumn{1}{c|}{Text} & LM & \multicolumn{1}{c|}{Model}& F1 & \multicolumn{1}{c|}{F1-label} & F1 & F1-label \\
\hlineB{2}
\multirow{3}{*}{ST} & \multirow{3}{*}{\cmark} & \multirow{3}{*}{\xmark} & \cmark & \xmark  & 67.4 & 76.3 & 68.0 & 77.1 \\
 & & & \xmark & \cmark  & 67.3 & 77.0 & \tba & \tba \\
 & & & \cmark & \cmark  & 70.6 & 79.9 & \tba & \tba \\
\hlineB{2}
\multirow{3}{*}{KD-ppl} & \multirow{3}{*}{\cmark} & \multirow{3}{*}{\xmark} & \cmark & \xmark  & 69.1 & 79.1 & 69.6 & 80.2 \\
 & & & \xmark & \cmark  & 70.9 & 83.2 & 74.3 & 83.9 \\
 & & & \cmark & \cmark  & 74.2 & 84.8 & 75.0 & 85.5 \\
\hlineB{2}
\multirow{3}{*}{KD-nlp} & \xmark & \cmark & \cmark & \xmark  & \tba & \tba & 71.7 & 80.9 \\
 & \multirow{2}{*}{\cmark} & \multirow{2}{*}{\cmark} & \xmark & \cmark  & 74.4 & 85.7 & 77.2 & 87.2 \\
 & & & \cmark & \cmark  & 79.2 & 87.4 & 81.8 & 89.0 \\
\hlineB{2}
ASR-NER & \cmark & \cmark & N/A & \cmark  & 70.7 & 80.5 & 73.2 & 81.9 \\
\hlineB{2}
\end{tabular}

\caption{Test set f-score (\%) performance for different methods of utilizing external data to improve E2E model. A ``\cmark'' for both speech and text external data implies presence of speech-text paired data. A ``\xmark'' for LM column implies no LM was used during decoding. ASR-NER model does not generate any new data for re-training LM, which is marked as ``N/A'' in the table, the numbers reported here are with LM decoding.}
\label{tab:all_res}
\end{table*}

==> tables/analysis.tex <==
% \begin{table*}[]
% \centering
% \begin{tabular}{c|cc|cc|cc|cc|cc}
% \hlineB{2}
% \multirow{2}{*}{Ext. data} & \multicolumn{2}{c|}{F1} & \multicolumn{2}{c|}{label-F1} & \multicolumn{2}{c|}{phrase-F1} & \multicolumn{2}{c|}{WER}  & \multicolumn{2}{c}{NE ACC} \\ \cline{2-11}
%                           & Pipeline     & E2E     & Pipeline        & E2E        & Pipeline     & E2E  & Pipeline & E2E & Pipeline & E2E    \\
%                           \hlineB{2}
% None & 72.0 & 68.1 & 84.2 & 76.7 & 73.6 & 69.0 & \tba & \tba & 81.9 & 80.4 \\
% Un-Sp                      & 74.9         & 77.0    & 85.8            & 85.7   & 76.2 & 77.4    & 10.63        & 11.90 & 84.4 & 83.5  \\
% Un-Txt                     & 73.1         & 71.3    & 85.1            & 79.8   & 74.3 & 72.6    & 11.97        & 13.37 & 81.9 & 83.1  \\
% Sp-Txt                     & 77.6        & 79.6    &87.9          & 87.4   & 79 & 81.0   & 9.61         & 10.25 & 88.7 & 90.7 \\
% \hline \hline
% text NER & \multicolumn{2}{c|}{86} & \multicolumn{2}{c|}{90.5} & \multicolumn{2}{c|}{88.8} & \multicolumn{2}{c|}{0}  & \multicolumn{2}{c}{100} \\
% \hlineB{2}
% \end{tabular}
% \caption{
% F1, label-F1, and word error rates on dev set for best performing models in each category with access to 100 hours of external data.\ap{I'll add NE-ACC here in the final version. Based on our current hypothesis, we expect NE-ACC for E2E to be higher than pipeline.}\ap{Scores in parenthesis are after combining the better trained asr with better self-trained ner text model: 77.0 (77.6),  87.9 (87.9), 78.7 (79) [76.8], 88.7 (88.7)}
% }
% \label{tab:analysis}
% \end{table*}

\begin{table*}[]
\centering
\begin{tabular}{c|cc|cc|cc}
\hlineB{2}
\multirow{2}{*}{Ext. data} & \multicolumn{2}{c|}{F1} & \multicolumn{2}{c|}{WER}  & \multicolumn{2}{c}{NE ACC} \\ \cline{2-7}
                           & Pipeline     & E2E   & Pipeline & E2E & Pipeline & E2E    \\
                           \hlineB{2}
None & 72.0 & 68.1  & \tba & \tba & 81.9 & 80.4 \\
Un-Sp                      & 74.9         & 77.0    & 10.63        & 11.90 & 84.4 & 83.5  \\
Un-Txt                     & 73.1         & 71.3    & 11.97        & 13.37 & 81.9 & 83.1  \\
Sp-Txt                     & 77.6        & 79.6    & 9.61 & 10.25 & 88.7 & 90.7 \\
\hline \hline
text NER & \multicolumn{2}{c|}{86} & \multicolumn{2}{c|}{0}  & \multicolumn{2}{c}{100} \\
\hlineB{2}
\end{tabular}
\caption{\ap{Will convert this into a graph representation.}F1, word error rate (WER), NE-ACC-detected on dev set for best performing models in each category with access to 100 hours of external data. The better performing approach within each row and metric-column is {\bf bold-faced}.
% F1, label-F1, and word error rates on dev set for best performing models in each category with access to 100 hours of external data.\ap{I'll add NE-ACC here in the final version. Based on our current hypothesis, we expect NE-ACC for E2E to be higher than pipeline.}\ap{Scores in parenthesis are after combining the better trained asr with better self-trained ner text model: 77.0 (77.6),  87.9 (87.9), 78.7 (79) [76.8], 88.7 (88.7)}
}
\label{tab:analysis}
\end{table*}

==> tables/effect-of-asr.tex <==
% \begin{table}[]
% \centering
% \begin{tabular}{c|cc|cc}
% \multirow{3}{*}{\# ASRdata} & \multicolumn{4}{c}{F-score}   \\
%                             & \multicolumn{2}{c}{2-stage} & \multicolumn{2}{c}{multi-task} \\
%                             & no LM      & 4-gram      & no LM        & 4-gram       \\ \hline
% None (from Tab.~\ref{tab:ssl})                       &    0.54 / 0.66        &  0.67 / 0.75              &              &                 \\ \hline
% 12h (matched)               &            &                &              &                 \\
% 100h                        &            &                &              &                 \\
% 500h                        &            &                &              &                
% \end{tabular}
% \caption{Effect of leveraging ASR data.\ap{We can decide to add only one of the two modeling techniques depending on what performs better and maybe mention the other in the text}\ap{Need to represent the pipeline model scores as well}}
% \label{tab:effect-of-asr}
% \end{table}

% \begin{table*}[]
% \centering
% \begin{tabular}{c|cc|cc}
% \multirow{2}{*}{\# data} & \multicolumn{2}{c|}{E2E} & \multicolumn{2}{c}{Pipeline}   \\ \cline{2-5}
%                             & no LM      & 4-gram LM      & no LM      & 4-gram LM \\ \hline
% None                       &    0.54 / 0.66        &  0.67 / 0.75     & - & -          \\ \hline
% 12h               &    0.55 / 0.68        &        0.67 / 0.76  & 0.49 / 0.72 & 0.7 / 0.82                 \\
% 100h                        &     0.61 / 0.72       &           0.70 / 0.78   & 0.65 / 0.82 &  0.75 / 0.86          \\
% 500h                        &      0.66 / 0.75      &     0.72 / 0.8                   & 0.69 / 0.83 & 0.78 / 0.87 
% \end{tabular}
% \caption{Test set \% f-score performance for ASR-NER models.\ap{Will clean this up; re-arrange columns and separate columns for F1 and label-F1}}
% \label{tab:effect-of-asr}
% \end{table*}

\begin{table*}[]
\centering
\begin{tabular}{c|c|cc|cc|cc|cc}
\hlineB{2}
\multicolumn{1}{c|}{\multirow{3}{*}{Model}} & \multicolumn{1}{c|}{\multirow{3}{*}{LM}} &\multicolumn{8}{c}{ASR pre-training data in ASR-NER models} \\
\cline{3-10}
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{2}{c|}{None} &\multicolumn{2}{c|}{15h} & \multicolumn{2}{c|}{100h} & \multicolumn{2}{c}{500h} \\
\cline{3-10}
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & F1 & label-F1 & F1 & label-F1 & F1 & label-F1 & F1 & label-F1 \\
\hlineB{2}
\multirow{2}{*}{E2E} & \xmark  & 50.2 & 64.0 & 51.9 & 65.8 & 59.6 & 70.7 & 61.8 & 72.9\\
 & \cmark & 63.4 & 71.7 & 64.1 & 72.1 & 65.7 & 74.6 & 67.1 & 76.2\\
\hlineB{2}
\multirow{2}{*}{Pipeline} & \xmark & \multicolumn{2}{c|}{\multirow{2}{*}{N/A}} & 46.4 & 70.7 & 60.8 & 78.6 & 65.4 & 79.8\\
 & \cmark & &  & 64.7 & 77.1 & 70.7 & 82.2 & 74.7 & 83.4\\
\hlineB{2}
\end{tabular}
\caption{Test set f-score (\%) performance for ASR-NER models.}
\label{tab:effect-of-asr}
\end{table*}

==> tables/effect-of-lm.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{c|cc|cc}
\hlineB{2}
Ext. data               & Method                            & LM        & \multicolumn{1}{c}{100h} & \multicolumn{1}{c}{500h} \\
\hlineB{2}
\multirow{6}{*}{Un-Sp}  & \multirow{3}{*}{SelfTrain-NER}    & no lm     &                          &                          \\
                        &                                   & 15h LM    &                          &                          \\
                        &                                   & plabel LM &                          &                          \\ \cline{2-5}
                        & \multirow{3}{*}{Distill-Pipeline} & no lm     &                          &                          \\
                        &                                   & 15h LM    &                          &                          \\
                        &                                   & plabel LM &                          &                          \\ \hlineB{}
\multirow{5}{*}{Sp-Txt} & \multirow{3}{*}{Distill-NLP}      & no lm     &                          &                          \\
                        &                                   & 15h LM    &                          &                          \\
                        &                                   & plabel LM &                          &                          \\ \cline{2-5}
                        & \multirow{2}{*}{Pre-ASR}          & no lm     &                          &                          \\
                        &                                   & 15h LM    &                          &                         \\
\hlineB{2}
\end{tabular}
\caption{Ablation study: Effect of LM \ap{Still debating whether to add both 15h and plabel LM}}
\label{tab:effect-of-lm}
\end{table}

==> tables/improve_ppl.tex <==
\begin{table*}[]
\centering
\begin{tabular}{lcc|cc|cc}
\hlineB{2}
\multicolumn{3}{c|}{Model} & \multicolumn{2}{c|}{External data type} & \multirow{2}{*}{SF1} & \multirow{2}{*}{label-F1} \\
\cline{1-5}
\multicolumn{1}{c}{Speech model} & LM & Text model & Speech & Text & &  \\
% \multicolumn{1}{c|}{\multirow{2}{*}{Speech model}}
% \multicolumn{1}{c}{Speech model} & \multirow{2}{*}{LM} & Text model & \multicolumn{2}{c|}{External data type} &F1 (\%) & label-F1 (\%)  \\
\hlineB{2} 
\textbf{NLP Topline:}  & & & & & & \\
\hspace{3mm} \multirow{1}{*}{ N/A (GT Text)} & \multirow{1}{*}{ N/A} & DeBERTa-B  & \na & \xmark & 81.4 & 86.3 \\
% & & DeBERTa-B+  & \na & \cmark & \tba & \tba \\
\hlineB{2}
\textbf{Pipeline approaches:}  & & & & & & \\
\hspace{2mm} W2V2-B & \xmark & DeBERTa-B & \xmark & \xmark & 49.5 & 74.2 \\
\hspace{2mm} W2V2-B+ & \xmark & DeBERTa-B & \cmark & \xmark& \tba & \tba \\
% \hspace{2mm} W2V2-B & \xmark & DeBERTa-B+ & \xmark & \cmark& \tba & \tba \\
% \hspace{2mm} W2V2-B+ & \xmark & DeBERTa-B+ & \cmark & \cmark& \tba & \tba \\
\hline
\hspace{2mm} W2V2-B & \cmark & DeBERTa-B & \xmark & \xmark& 49.5 & 74.2 \\
\hspace{2mm} W2V2-B+ & \cmark & DeBERTa-B & \cmark & \xmark& \tba & \tba \\
% \hspace{2mm} W2V2-B & \cmark & DeBERTa-B+ & \xmark & \cmark& \tba & \tba \\
% \hspace{2mm} W2V2-B+ & \cmark & DeBERTa-B+ & \cmark & \cmark& \tba & \tba \\
\hlineB{2}
\end{tabular}
\vspace{-2mm}
\caption{Improvement from self-training for the pipeline models.}
\vspace{-4mm}
\label{tab:ner_task_detail}
\end{table*}


==> tables/key-results.tex <==
\begin{table}[]
\centering
\begin{tabular}{c|cc|cc}
\hlineB{2}
\multirow{2}{*}{Ext. data} & \multicolumn{2}{c|}{100h} & \multicolumn{2}{c}{500h}                       \\
                                    & Pipeline      & E2E      & Pipeline             & \multicolumn{1}{c}{E2E} \\ \hlineB{2}
None                                &               &          & \multicolumn{1}{l}{} &                         \\
Un-Sp                               &               &          & \multicolumn{1}{l}{} &                         \\
Un-Txt                              &               &          &                      &                         \\
Sp-Txt                              &               &          &                      &                         \\ \hlineB{2}
\end{tabular}
\caption{\ap{These will have select numbers from Tables~\ref{tab:results-e2e} and \ref{tab:results-ppl}. Considering presenting this as a plot instead} Key results from the experiments leveraging different combinations of 100h and 500h of external data. The E2E experiments for unlabeled speech and speech-text pairs are performing using knowledge-distillation from pipeline and text NER models respectively. The rest use the approaches mentioned in section~\ref{tba}}
\label{tab:key-results}
\end{table}

==> tables/self-training.tex <==
% \begin{table}[]
% \centering
% \begin{tabular}{cc|c}
%                                          & iter & F-score \\ \hline
% w2v2-ls-12h (from Tab.~\ref{tab:effect-of-asr})                  & n/a  &         \\ \hline
% \multirow{2}{*}{+488h speech (E2E)}      & 0    &         \\
%                                          & 1    &         \\ \hline
% \multirow{2}{*}{+488h speech (pipeline)} & 0    &         \\ 
%                                          & 1    &         \\ \hline
% \multirow{2}{*}{+488h text (NLP)} & 0    &         \\ 
%                                          & 1    &         \\         
% \end{tabular}
% \caption{Leveraging unlabeled text/speech modalities; $k=1$ \ap{or 2?} \ap{For the unlabeled speech we can either use the pipeline or the E2E model to generate pseudo-labels. Note to mention which we did and why.}}
% \label{tab:self-training}
% \end{table}


% \begin{table}[]
% \centering
% \begin{tabular}{cc|cc}
% Model &  & \multicolumn{2}{c}{F-score} \\ \hline
% w2v2-ls-12h & & \multicolumn{2}{c}{0.67 / 0.76} \\ \hline
%                                   & iter & 100h         & 500h         \\ \hline
% \multirow{2}{*}{speech (E2E)}      & 0    &     \tba         &    0.67 / 0.75          \\
%                                   & 1    &      \tba        &   0.71 / 0.78           \\ \hline
% \multirow{2}{*}{speech (pipeline)} & 0    &       \tba       &    0.69 / 0.78          \\
%                                   & 1    &       \tba      &   \tba           \\ \hline
% \multirow{2}{*}{text (nlp)}        & 0    &       \tba       &    0.71 / 0.79          \\
%                                   & 1    &     \tba         &    \tba         
% \end{tabular}
% \caption{Leveraging unlabeled text/speech modalities}
% \label{tab:self-training}
% \end{table}

==> tables/ssl.tex <==
% \begin{table}[]
% \centering
% \begin{tabular}{c|cc}
%                               & \multicolumn{2}{c}{F-score}                 \\
%                               & no LM                & 4-gram LM            \\ \hline
% Baseline                      &   \tba                   &    \tba                  \\ \hline
% w2v2-multi-10k                &  0.50 / 0.60                    &     0.64 / 0.70                 \\
% w2v2-multi-100k               &      0.52 / 0.63                &     0.66 / 0.73                 \\
% w2v2-ls                       &       0.54 / 0.66               &        0.67 / 0.75              \\
% hubert-ls                       &         0.53 / 0.66             &        0.67 / 0.74              \\
% \end{tabular}
% \caption{Effect of self-supervised pre-training with and without using LM for decoding. Baseline model here does not leverage any unlabeled speech data. (i) NE-ACC: fraction of named entities correctly decoded, (ii) NE-WER: WER of NER annotated text, (iii) F-score: evaluates (entity phrase, entity tag) pairs.}
% \label{tab:ssl}
% \end{table}
